"For Us By Us": Intentionally Designing Technology for Lived Black Experiences

HCI research to date has only scratched the surface of the unique approaches racially minoritized communities take to building, designing, and using technology systems. While there has been an increase in understanding how people across racial groups create community across different platforms, there is still a lack of studies that explicitly center on how Black technologists design with and for their own communities. In this paper, we present findings from a series of semi-structured interviews with Black technologists who have used, created, or curated resources to support lived Black experiences. From their experiences, we find a multifaceted approach to design as a means of survival, to stay connected, for cultural significance, and to bask in celebratory joy. Further, we provide considerations that emphasize the need for centering lived Black experiences in design and share approaches that can empower the broader research community to conduct further inquiries into design focused on those in the margins.

==> alttext.tex <==
Icons: [Project icons are as follows: Resource is associated with an icon of a book, tool is associated with an icon of a wrench, community is associated with an icon of two people standing facing each other with a doubled sided arrow in between them, and service is an icon of a market stand.]


Table 1: [Description of Black & Non-Black Technologists with Project Type: categorized by Resource, Tool, Community, or Service. The first column is titled PID and contains the participant ID numbers, the second column is titled project description and contains descriptions of each participant’s projects, and the third column is titled project type and contains the icon associated with the project type.]

Table 2: [Core Categories Of What It Means To Design For The Black Experience. First Column Is Titled “Core Category”, Second Column Is Titled “Category Description” And Third Is “Aligned Projects”]

